Report on the First HIPstIR Workshop on the Future of Information Retrieval

The vision of HIPstIR is that early stage information retrieval (IR) researchers get together to develop a future for non-mainstream ideas and research agendas in IR. The first iteration of this vision materialized in the form of a three day workshop in Portsmouth, New Hampshire attended by 24 researchers across academia and industry. Attendees pre-submitted one or more topics that they want to pitch at the meeting. Then over the three days during the workshop, we self-organized into groups and worked on six specific proposals of common interest. In this report, we present an overview of the workshop and brief summaries of the six proposals that resulted from the workshop.

==> 04-pitch.tex <==
\section{Summary of seed pitches}
\label{sec:pitch}

All attendees were encouraged to pre-submit one or more topics that they want to pitch at the meeting.
A compiled list of all pre-submitted pitches is presented below.

\subsection{People, real systems, real constraints \\
{\footnotesize by Adam Roegiest}}

Generally, IR has focused on a fixed set of similar tasks and has explored them in-depth with user models and simulations.
There has also been much exploration of efficiently utilizing CPU/RAM to aid retrieval times.
But much of the real-world exists with many non-experts using systems designed by experts in the field to do some non-standard IR tasks.
Moreover, there are often constraints that can meaningfully change system design and implementations to accommodate regulatory requirements and similar constraints.
For example, in eDiscovery, systems and models may be tailored to a single case and then discarded.
Such systems may also have novel interactions that don't fit into more commonly examined tasks.
Similarly, in Due Diligence contexts, there must be tight controls one which lawyers have access to which documents to avoid conflicts of interest.

Accommodating these different constraints for different real-world problems impose changes on user models and interactions that may not be explained under current IR models.

Moreover, ensuring that users are able to adequately understand why certain information was or was not provided/returned by a system may also impose restrictions on the types of systems that can be designed.
Such explanations may be required due to legal, regulatory, or compliance reasons.
 
The pitch boils down to bringing all sides together (industry, academia, and subject matter experts, and others) to find innovative and creative solutions to problems that people face everyday but do not get the same ``love'' by researchers that is paid to traditional IR tasks.

\paragraph{List of Papers and Explanations}

\begin{description}[leftmargin=0.13in]

\item [\citet{amershi2019guidelines}.]
As we progress to include more ML/AI into our systems, how we navigate the interactions between these components and the users becomes critically important.
Partly because there are likely going to be increasing requirements to know/understand/explain the decisions these components make; and partly because these interactions govern how well the components perform and how much utility that users can get out of the platform.
We have seen the latter with our in-house former lawyers who use our system in their day-to-day.
Accordingly, setting up good guidelines/best practices for interaction may help mitigate inconsistencies between systems.

\item [\citet{wei2019bubbles}.]
Essentially, this provides an example of making the experience real for users.
In particular, in how we can align these complex retrieval systems to users' mental models to help aid how they interact and interpret the systems' results.

\item [\citet{scholtes2013impact}.]
The point of this paper is to highlight that the operational environments of systems in situ does not always reflect that of academic research.
In this case, the paper reports on problems caused when document collections are grown over time in the eDiscovery setting.
But this can manifest in other ways, such as documents being segregated from some users to avoid conflicts of interest or regulatory compliance that requires documents to be deleted after some point.
There may even be more subtle constraints that restrict how system results or ML models can be shared (e.g., between law firms or even partnered law firms).
The intent here is to provide some additional colour into the ``real constraints'' aspect of the abstract.

\end{description}

\subsection{Democracy in danger: controversy, polarization, disinformation, and botnets \\
{\footnotesize by Shiri Dori-Hacohen}}

The institution of democracy is currently at risk in the form of botnets and disinformation (as opposed to the frivolous accusation of fake news, which is lobbed at real journalism in order to delegitimize it).
Regardless of our political beliefs or nationalities, the Mueller report confirms that Russia successfully interfered with the 2016 U.S.
election by intentionally polarizing the U.S.
population via the successful and targeted use of fake personas and botnets to create divisiveness on highly controversial and charged topics.
It may not be an exaggeration to say that addressing this problem may slow or stop the world's dangerous slide into populism and violence.

\paragraph{List of Papers and Explanations}

\begin{description}[leftmargin=0.13in]

\item [\citet{vicario2019polarization}.]
An attempt to predict which topics are more likely to be targeted by disinformation.

\item [\citet{kaplun2018controversy}.]
A formalized attempt to connect sentiment and controversy, which have been previously demonstrated to be uncorrelated.

\item [\citet{sznajder2019controversy}.]
A new approach to detecting controversy levels.

\item [\citet{bennett2018disinformation}.]
From the Social Sciences---but strongly supports the pitch.
A paper directly connecting disinformation to the intentional disruption of democratic institutions.

\end{description}

\subsection{Establishing an exchange rate between implicitly-collected and explicitly-given user data \\
{\footnotesize by Jeremy Pickens}}

At the risk of painting with too broad of a brush stroke, core IR ranking algorithms---that is to say ranking algorithms relying only on the statistics of a collection itself and not user interaction data (log files) -- have not improved in quite some time.
Most if not all improvements have come in the form of some amount of implicitly-collected user data, \eg, log files of general historical user search interactions, or personalization in the form of implicitly collecting private user data such as location, previous search history, or possibly other demographic information.

At the same time, it has long been known that explicit user interaction yields excellent results as well.
A user marking a document as relevant provides a much stronger signal than a click.
A user using explicit operators, such as site: or (file)type: is a much clearer declaration of user intent, and better results will often follow as well.
System improvements can be garnered via both methods: implicitly-collected and explicitly-given.

So the question is: How much implicitly-gathered data needs to be collected to result in a quality improvement equal to explicitly-given data?  Or, stated another way, if search engines stopped collecting and using implicit data, how much explicit user effort would be required to achieve a similar result quality? 

What is the exchange rate?
This question of exchange rate is an interesting one, because implicitly collected data is often extracted from users without their knowledge or permission.
That is to say, privacy lines are often crossed.
If explicitly-given data were to have a favorable ``exchange rate'' with implicitly collected data, that explicit data would not have to be stored by the search engine.
It could be given by the user in the moment, and then forgotten as quickly as it was used.
A search engine based on explicit feedback could therefore allow the user to trade ease of use for increased privacy, and vice versa.

But that is only possible if IR system designers have a good sense of the exchange rate between implicitly-collected and explicitly-given user data.

\subsection{Information retrieval with human-out-of-the-loop \\
{\footnotesize by Bhaskar Mitra}}
Many information retrieval (IR) systems presupposes interaction with a human end-user.
This assumption is ingrained in many aspects of these systems’ designs—from assuming short sequences of keywords as representation of information needs to ranked list of information artifacts as the preferred presentation scheme for retrieved results.
For our users, however, the act of searching is often a support for a larger task (e.g., planning a vacation, working on a project).
As machine learning (ML) and artificial intelligence (AI) find more creative applications in assisting human users with these tasks, a likely scenario arises in which it is the ML/AI application that interfaces with the IR system and not the user.
This creates a unique opportunity to rethink the design of our IR systems considering the end user to be an autonomous ML/AI agent.

Several recent papers on conversational AI agents (Ghazvininejad, et al., 2018, Dinan, et al., 2018), for example, have incorporated IR sub-systems.
The IR sub-systems in these cases typically comprise of simple term matching (e.g., BM25) or nearest-neighbour search in a learned embedding space—followed by a re-ranking stage and/or the application of attention mechanisms over the top K retrieved items.
It is likely that we can improve upon these IR models—that have historically evolved under the assumption of a human end-user—by relaxing on those very constraints.
What is the ``best'' query to express an information need, if we do not assume a user who is reluctant to type any more than a few terms into the search box? What information should the retrieval system produce in response when not optimizing for inspection by an end user who is unlikely to scroll down a long list? How should we redesign the metrics we optimize for? How should the retrieval function and corresponding data structures evolve under these new assumptions? These are some of the many interesting research questions that we must address as part of this proposal.

The application of ML/AI for IR tasks have garnered significant attention in recent years.
In contrast, this proposal encourages the exploration of IR methodologies for ML/AI applications.
To misappropriate the John F. Kennedy quote: ``\emph{Ask not (only) what machine learning can do for IR, ask what IR can do for machine learning}''.

\paragraph{List of Papers and Explanations}

\begin{description}[leftmargin=0.13in]

\item [\citet{ghazvininejad2018knowledge}, \citet{dinan2018wizard}.]
Both papers above incorporate IR sub-systems into conversational / dialogue generation models.

\item [\citet{nogueira2017task}.]
This line of work on learning to formulate queries assuming a specific retrieval system may be relevant the context of agents learning to express their information needs.

\end{description}

\subsection{The entire history of you: retrieval models for visual lifelog collections \\
{\footnotesize by Bhaskar Mitra}}
The third episode of British science fiction anthology series Black Mirror (season 1)—titled ``The entire history of you''—describe a fictional implant that enables subjects to record and playback their personal audio-visual memories.
This notion of ``lifelogging'' has, in fact, been studied extensively in the literature (see: Gurrin et al., 2014, Sellen and Whittaker, 2010) and poses interesting opportunities.
Imagine being at the grocery store and being able to quickly retrieve a visual entry from your personal lifelog to figure out if you should buy more milk—or being in the middle of a conversation and quickly referencing your visual lifelog for the name of the restaurant you were at last week (whose name seems to escape you this very moment).

However, as Gurrin et al. (2014) point out that there has been limited development in lifelog retrieval models.
We hypothesize that this is at least partially due to the limited effectiveness of state-of-the-art models for automatic object recognition and image/video representation learning at that time.
There have been significant developments in the capabilities of deep models for computer vision in the last half a decade—and what may have been pure science fiction then may be much more plausible today.

So, towards that goal, we envision a simple study: let a subject watch a movie/video and then answer specific questions while having access to the video—directly or via an IR system.
For example, say the subject watches ``When Harry met Sally'' and is then required to answer ``what was Harry Burns (Billy Crystal) wearing in the Katz's Delicatessen scene?'' (the correct answer being a gray & brown jumper).
Our goal would be to design an IR system that minimizes the time and effort required to complete the task.
We pose no constraints on the design or interface of the IR system—e.g., the interface may be search-based or a browse-based, the interaction may involve single or multiple turns, may or may not involve text based input/output.

The idea of being able to log and search/browse one’s personal memory is a grand objective.
However, we must recognize the irony in taking our motivation from a television show about technological dystopia—which is meant to serve as a cautionary tail of unintended social consequences of unfettered pursuit of technology.
It is therefore, important that we highlight that to build such a technology would require not just progress in retrieval models, but also significant research, grounded in ethical and social science studies, to understand the impact—for both the society and the individual—with respect to privacy, law, and human rights as a consequence of ``never forgetting''.

\paragraph{List of Papers and Explanations}

\begin{description}[leftmargin=0.13in]

\item [\citet{gurrin2014lifelogging}.]
A survey of lifelogging literature.

\item [\citet{sellen2010beyond}.]
A piece that is critical of the impact lifelogging in its current state.
It would be important to understand the shortcomings and the gaps that needs to be filled.

\item [\citet{dumais2016stuff}.]
Describes the design and evaluation of an IR system that builds a unified index of diverse information artifacts (e.g., email, documents) the user has viewed in the past.

\end{description}

\subsection{Making automated pipelines semi-automated with interactive IR \\
{\footnotesize by Henry Field}}
There are many complex tasks (within and outside of IR) for which a human could perform the entire operation manually, but it takes too much time or effort.
Fully automated solutions save time, but aren't always as accurate as desired, sometimes due to the propagation and amplification of errors during the processing pipeline or a mismatch in user intent.
Can we find a way to achieve higher accuracy and lower human effort? One potential approach is to find the decision points in the underlying processes that lend themselves to human feedback.
While I have a particular example in mind, I imagine that it is generally (or at least often) the case that the options at these decision points can be extracted, contextualized, and ranked.
In fact, even the set of decision points could be ranked/prioritized based on the potential impact that human feedback may have on the remainder of the process (as is done in some semi-supervised machine learning).

The interactive IR components to this are: extracting and ranking options, visualizing the options, and the UX of the whole thing, including contextualizing the decision points and options.
Generalizing these so they can be applied to a wide variety of tasks should also be explored.

Here's the particular example I have in mind.
In his PhD thesis ``Social Network Extraction from Text'', Agarwal (2016) describes a full pipeline for extracting character networks from plain text novels.
This involves a number of smaller steps, including identifying the characters and their aliases, their mentions, whether there is a relationship between two characters, and what that relationship is.
There are many places where this pipeline can go astray and the results are lower than ideal accuracy.
For example, suppose this pipeline erroneously conflates two characters (e.g., Bob and Robert); this will impact the remainder of the pipeline.
To mitigate this, we could present a human familiar with the book with a list of characters and their aliases and ask them to edit the list as necessary, highlighting low confidence aliases and suggesting alternative groupings.
Now suppose the algorithm fails to resolve a pronoun correctly.
We could allow the human to click on the pronoun in the text and select alternatives from a ranked list of characters the pronoun might refer to.
Correcting these errors should have a substantial positive impact on the final accuracy of the pipeline, while requiring a (hopefully significantly) smaller amount of human intervention than annotating the text manually (which is the approach taken by some literary scholars).

Some other examples of tasks that might benefit from this: relevance feedback (e.g., allow users to see and modify the relevant documents/parts of documents), product/song/video recommendation (e.g., allow the user to remove previously viewed items that are out of context or irrelevant), and personalization.

\subsection{Evaluating IR systems from a user perspective \\
{\footnotesize by Widad Machmouchi}}
While there are multiple measures for how successful IR systems are, they mostly rely on labels collected from judgments trying to replicate the user experience.
Such measures are great as ``inner loop'' metrics, where the researcher is refining their solution, but the litmus test for a good IR system is whether it is satisfying its users' needs.
I would like to see more solutions put through experiments with real users to properly evaluate the improvement they introduce to the user experience.

\subsection{Scientific diligence from IR \& ML tools \\
{\footnotesize by John Foley}}
There are a wide variety of IR \& machine learning tools and toolkits out there: Indri, Galago, Terrier, Ranklib, RankSVM, Liblinear, LibSVM, Tensorflow, Pytorch, xgboost, trec\_eval, etc.
And none of their output is close to be ready to be put in a published paper without a vast amount of time-consuming and error-prone work.

In fact, of the list above, only Ranklib has any support for cross-validation.
When such tools are provided, they are always opt-in, not opt-out.
None of these tools provide confidence intervals on standard evaluation metrics or make significance testing part of the pipeline.

It is entirely unethical to be using or creating tools that provide single point estimates of performance.
If we don't want another decade of ``improvements that don't add up'' we need to change the culture; and that starts with our tools saying ``maybe'' and ``no significant difference'' in the appropriate amounts, and automatically performing as much statistical analysis as is possible, and ends with tools that are more robust to errors in post-analysis because they *always* perform re-sampling and cross-validation experiments.

We know how to do significance testing and construct confidence intervals for our favorite measures: (e.g., \citep{park2011bootstrap}.)

We should get the field toward pre-registration of hypotheses (https://cos.io/prereg/)

But there's low-hanging-fruit that we could use to make this less of a cultural/individual-effort problem.

\paragraph{List of Papers and Explanations}

\begin{description}[leftmargin=0.13in]

\item [\citet{strubell2019energy}.]
It is not clear to me that the field is making progress, and we need to change the way we perform and evaluate research.
We need new datasets on new problems to succeed, and we can't ignore strong baselines (have you tried a linear model recently?) because they don't fit our idea of what a new paper should be.

\end{description}

\subsection{Explaining search results \\
{\footnotesize by Adrian Boteanu}}
Aided by knowledge graphs, search engines are starting to supplement search results with additional structured data, for example an author’s recent books and place of birth.
This is in line with the assumption of traditional IR, that users will know how to interpret the results.
However, relaying results to users is particularly challenging when answers are available in semi-structured formats, when explanation templates are insufficient and the results may require time to read.
Similarly, evaluation benchmarks in IR have focused on ranking results, without taking into consideration how these results are presented, for example the degree of summarization.

\subsection{On the impacts of IR systems on their users \\
{\footnotesize by Asia Biega}}
Responsible data science is becoming a very active research area, broadly focusing on the issues of fairness, ethics, privacy,  and the influence of socio-technical systems on societies.
While much work to date has been devoted to the impacts of systems on groups of people and large-scale processes surrounding them, the impacts of systems on individuals remain largely under-explored.
In light of the emerging well-being movements and initiatives such as 'Time well spent' of the Centre for Humane Technology, it is pertinent to ask how systems might manipulate user behavior and beliefs, limit individual freedom and agency, or diminish overall user well-being.
The information retrieval community is well-geared for tackling these problems, given its expertise in studying the interactions between users and systems.

\paragraph{List of Papers and Explanations}

\begin{description}[leftmargin=0.13in]

\item [\citet{schneider2018digital}.]
An overview of how people's behavior can be influenced using simple interface interventions.

\item [\citet{kaptein2010selecting}.]
A discussion of how recommender systems can leverage so-called persuasion profiles to manipulate users.

\end{description}

\subsection{Preference elicitation and system initiative to support collaborative information-seeking \\
{\footnotesize by Sandeep Avula}}
Imagine standing by the kitchen counter and discussing the upcoming dinner party with your partner.
While you could individually look up for ideas on your personal devices, I urge you to imagine a scenario where you both could consult a system, together, for ideas.
This system could be a proxy for a friend who is a Michelin star chef and also knows the limits of your cooking abilities.
This system could elicit your preferences and then try to suggest menus, and in the event you get ambitious, ask you to hold back.
While such a system elicits your preferences, it must be aware of when to ask, so that it may not interrupt your conversation, and also which type of question to ask.
While the subject of preference elicitation has received good attention in recent times, this has been generally studied in a single user setting.
Next, there is also little understanding of when a system should take the initiative in information-seeking dialogues.
Understanding both elicitation and system initiative in a collaborative setting are crucial to developing a system that we can embed into people’s everyday lives.
In this workshop, WE hope to encourage conversations on study designs, which will allow us to understand how conversational search systems must operate in multi-user scenarios.

\paragraph{List of Papers and Explanations}

\begin{description}[leftmargin=0.13in]

\item [\citet{radlinski2017theoretical}.]
This paper gives us a framework to think about conversational search.
It discusses about the different functionalities a system should support.
Two of which that are related to my pitch are system initiative and preference elicitation.

\item [\citet{avula2018searchbots}.]
This paper deals with embedding search tools into a conversational platforms.
This is a Wizard of Oz study, where in a structured format, the Wizard elicits preferences from the users.
While the users perceive benefits of such elicitation, they also report their frustration with the ``timing'' of the intervention.

\item [\citet{seering2019beyond}.]
This paper explores chatbots beyond typical one-on-one settings.
They discuss the social implications and the roles that bots have when participating with multiple users.

\end{description}

\subsection{Hardware for natural language processing (NLP) \\
{\footnotesize by Alexandre Tachard Passos}}
GPUs, TPUs, and all the mobile-specific hardware coming out tends to be designed with computer vision in mind first and foremost.
Then NLP models are developed to leverage this hardware's characteristics (transformers being more amenable to parallelism and large-batch training than LSTMs being an example).
What would it take to make hardware that would actually prioritize NLP? And how would the ideal way of programming this hardware differ from the very rectangular-array-focused libraries we have today for PyTorch, TensorFlow, JAX, \etc?

\subsection{Reproducibility in IR \\
{\footnotesize by Matthew Mitsui}}
With the replication crisis being a hot discussion topic in the social and hard sciences, reproducibility has inevitably made its way into discussion circles in the information retrieval (IR) research community.
The ACM has initiated a policy for badging papers that hit certain milestones for reproducibility and replicability.
In addition, the SIGIR community has organized workshops such as the Open-Source IR Replicability Challenge (OSIRRC) and the Barriers to Interactive IR Resources Re-use (BIIRRR) workshop.

We start by discussing the approaches taken in some other fields to promote reproducibility, highlighting the challenges faced in these implementations.
We open the floor to discussing whether and how the IR community will face similar challenges, for the purpose of addressing whether/how our current efforts will solve our reproducibility challenges.
Relevant subtopics include but are not limited to: privacy in data sharing, what tools and environments can help facilitate reproducibility, solutions in an interdisciplinary environment, and whether positive badging is useful/enough.

\paragraph{List of Papers and Explanations}

\begin{description}[leftmargin=0.13in]

\item [\citet{ferro2018sigir}.]
The SIGIR report on the ACM badging initiative, for the uninitiated.
This overviews the types of badges, as well as the efforts that will be implemented in SIGIR, specifically a task force.

\item [\citet{sakai2016statistical}.]
A SIGIR 2016 paper indicating that several TOIS  papers from 2006-2015 are underpowered, overpowered, or do not indicate significance testing, which can affect meta-analyses and indicate other reproducibility issues.

\item [\citet{claesen2019preregistration}.]
Some reproducibility efforts may not produce the desired behavioral change---in this case, pre-registration.
27 examined papers deviated from their plan at time of pre-registration.
Deviations include: Hypotheses/RQs, variables, direction of effect, sample size collected, and statistical model used.

\item [\citet{soltani2019coagmento}.]
We see one side of the reproducibility coin as reducing the bottleneck from research idea to research product---\eg, a conference paper.
We repurposed a tool called Coagmento with this philosophy in mind.

\end{description}

\subsection{Multi-modal conversational search and recommendation leveraging deep domain understanding \\
{\footnotesize by Jeff Dalton}}
Over the next three to five years there will be a major change in search and recommendation systems to leverage conversational interaction in fundamentally new ways.
We propose that multi-modal conversational systems that leverage voice, text, video, and other forms of machine perception (including possibly computational smelling and eating).
 To be effective we propose that the models must be built on and effectively incorporate deep domain knowledge---the form and nature of how to do create, represent, and compute over this knowledge is an open problem.
The systems will also push the boundaries of multi-modal interaction in a conversational context with systems taking initiative and proactively starting conversations, use richer user models, improved simulation and new agent optimization methods (possibly building on reinforcement and inverse learning), and others.

\paragraph{List of Papers and Explanations}

\begin{description}[leftmargin=0.13in]

\item [\citet{kaiser2017one}.]
An early attempt to train a single multimodal model across domains: speech, translation, image, \etc spanning domains and modalities.
This hints at more recent work, like VisualBert.

\item [\citet{angeli2016combining}.]
Conversational systems need to scalably acquire deeper domain knowledge.
This is an interesting perspective of attempts in the NLP community based on Natural Logic.
In particular interesting is development towards gameplaying and simulation.
It's related to \citep{chen2017reading}.

\item [\citet{szlam2019build}.]
This is a recent position paper that argues for embedding an assistant in a game interface and using natural language presents unique opportunities.

\item [\citet{strub2017end}.]
This paper continue an important goal of multimodal visually grounded dialog systems combined with end-to-end learning based on RL.

\item [\citet{allen2019challenge}.]
A discussion on the future of dialogue systems from leaders in the field across diverse subtopics in the target pitch area.

\end{description}

\subsection{From query to model: information retrieval as a foundational technology for the humanities and social sciences \\
{\footnotesize by David Smith}}
The digital humanities (DH) and computational social sciences have focused much of their methodological discussion on hypothesis testing and causal inference.
 These fields, however, owe much of their progress to date to fairly generic information retrieval models.
 Many inference tasks---from detecting political events, classifying images of protests, tracking characters in films, transcribing manuscripts, and recognizing plot tropes---are justified by their use in retrieval systems.
 Particularly in DH, multi-year projects often focus on building retrieval systems.
 These fields provide opportunities for IR research in user studies, evaluations, models, and systems to bridge the gap between keyword search and confirmatory modeling for communities of expert and casual users.

\paragraph{List of Papers and Explanations}

\begin{description}[leftmargin=0.13in]

\item [\citet{underwood2014theorizing}.]
This paper makes the case that the fundamental enabling technology for the digital humanities and computational social sciences is information retrieval.
But if search is so central, why not think about different models and tasks.

\item [\citet{king2017computer}.]
This paper by three political scientists will probably be a bit infuriating to IR researchers, since it misdefines unsupervised learning and reinvents and then dismisses IR work on relevance feedback.
But it tries to grapple, somewhat, with the problems of exploratory data analysis in the social sciences and the interleaved tasks of retrieving individual documents and defining reference collections.
Another important topic for IR in the humanities and social sciences is the focus that history and archival studies places on provenance and source criticism (Quellenkritik).
Many existing digital collections are not associated with a reliable chain of custody; however, helping scholars to make inferences about sources then becomes an additional useful task.

\end{description}

\subsection{Constructing answers and generating information objects \\
{\footnotesize by Laura Dietz}}
Search result rankings are not ideal for many use cases, especially for diffuse and open information needs, or information needs a user does not know much about, or other information needs usually associated with exploratory search.
In such cases, rather than displaying a ranking of raw data, it would be better to process the information, determine what is most relevant, identify topics, consolidate common themes  and provide an aggregate summary of the information.

We have been studying this inter-disciplinary area between IR, NLP, KDD, and AKBC in the context of the TREC Complex Answer Retrieval  in the last few years.
Here given a title and an outline of a topics, the task is to generate a Wiki-like article on the topic.

The newly introduced TREC Conversational Assistance track casts this problem with an emphasis on a multi-turn conversation.

The SWIRL III \citep{culpepper2018research} describes this problem in more general terms in Chapter 7 on Generated Information Objects (GIOs).

There are not only many tasks and directions to be explored, but we can also imagine a wide variety of applications that share the same underlying research need.

\subsection{Better candidate set retrieval \\
{\footnotesize by Jordan Ramsdell}}
For many retrieval tasks, it is computationally infeasible to evaluate the relevance of all documents in a database given a query.
Typically one instead retrieves a subset of candidate documents using a less expensive method, such as BM25, and then evaluates this subset using a more expensive method (such as a neural network).
The drawback of this approach is that if a candidate set contains few relevant documents, there is not much one can do to improve performance without having to retrieve a better set.

Ideally, we would rather use our more expensive (and hopefully better!) method to retrieve documents.
How can we approximate such methods so that we can use them to evaluate all documents in a corpus? Can we also do a better job at picking subsets for evaluation? While these questions aren't new, answers to them could result in a general improvement to just about any retrieval method that depends on a candidate set, so they are worth exploring more extensively.

\subsection{Quantum-like language model and its applications \\
{\footnotesize by Sumanta Kashyapi}}
In recent times there have been many significant efforts to incorporate various concepts of quantum probability theory into some aspects of Information Retrieval research.
In some specific problem settings quantum inspired language models show significant improvement.
In coming years we expect to gain deeper insight into the interaction between building blocks of language when seen through the perspective of a quantum theorist.

\paragraph{List of Papers and Explanations}

\begin{description}[leftmargin=0.13in]

\item [\citet{zhang2018end}.]
This paper shows quantum inspired language model combined with neural architecture contributes to better performance in question answering task.

\item [\citet{sordoni2013modeling}.]
A generalized language model is developed using the probabilistic framework of quantum theory.
The authors show that this model outperforms a robust bag of words and another stronger non-bag of words baseline.

\item [\citet{li2016adaptive}.]
In this paper the authors demonstrate how Quantum Language Model can be utilized in modeling the complex term dependencies and continuously evolving information need of a user during a search session.

\end{description}

\subsection{Integrating passage and entity features for better passage retrieval \\
{\footnotesize by Shubham Chatterjee}}
Passage retrieval and Entity retrieval are well studied information retrieval tasks and various approaches have been taken in literature for each task separately.
While each passage/entity retrieval methods provides valuable information individually, it would be interesting to see how integrating these features help in passage retrieval.
While passage features provide coarse grained knowledge,  entity features provide fine grained knowledge, and their amalgamation might help in better passage retrieval.

\paragraph{List of Papers and Explanations}

\begin{description}[leftmargin=0.13in]

\item [\citet{sanz2019information}.]
The fast growth and development of online social networks has posed new challenges for information retrieval and, as a particular case, recommender systems.
A particularly compelling problem in this context is recommending network edges, that is, automatically predicting people that a given user may wish or benefit from connecting to in the network.
This task has interesting particularities compared to more traditional recommendation domains, a salient one being that recommended items belong to the same space as the users they are recommended to.


\item [\citet{osche2019antrs}.]
When people use recommender systems, they generally expect coherent lists of items.
Depending on the application domain, it can be a playlist of songs they are likely to enjoy in their favorite online music service, a set of educational resources to acquire new competencies through an intelligent tutoring system, or a sequence of exhibits to discover from an adaptive mobile museum guide.
To make these lists coherent from the users’ perspective, recommendations must find the best compromise between multiple objectives (best possible precision, need for diversity and novelty).

\end{description}

\subsection{Behavioral context influence on product assessments \\
{\footnotesize by Hanaa Anber}}
Often times, products or services critiques stem from physical flaws or personal bad experiences which leave obvious clues for improvements.

Other times, critiques could be influenced by poor positioning of the product or service through mismatched marketing conditions.
In this instance, though with less obvious clues, refinements are still conceivable.

However, in not uncommon times, critiques are decided upon by external factors, outside the realm of the product or service itself, that could be flawless.

Those include emotional critiques driven by extrinsic (pleasant or unpleasant) incidents, or irrational assessments influenced by peer-expectations or even monetary incentives.
In this case, analysis of the consumer historical behavior (on social media, for example) is necessary to distill ratings validity.

\paragraph{List of Papers and Explanations}

\begin{description}[leftmargin=0.13in]

\item [\citet{liu2016pt}.]
This paper proposes a new model to predict personality traits on social media.
That model is an extension of ``Latent Dirichlet Allocation Model''.
In the results, they showed a new method to uncover human behavior on social media by extracting the interpretable topics, which is associated with each personality trait.

\end{description}

\subsection{Close domain NLP + multilingual NLP \\
{\footnotesize by Palliika Kanani}}
There is a lot of progress in general language understanding (and IR).
However, as AI is being adopted more broadly by various industries, applying these technologies to specialized domains still remains a challenge.
Think law, banking, manufacturing, customer service for specific types of businesses and so on.
The progress in transfer learning technologies have also helped significantly in reducing the need for large amounts of domain specific training data, but the effectiveness of these approaches for niche domains is still questionable.
A related area is understanding short, noisy pieces of text out of context, these include text snippets found in industrial settings, such as parts of business documents or product descriptions, etc.
Again, translating the gains in general language understanding for these domains needs more work.

Despite recent advances, there is need for additional focus on Multi-lingual NLP, especially for languages with lower resource availability.


==> 10-recipe.tex <==

\section{Appendix: Recipe to bake your own HIPstIR}

Ingredients:
\begin{itemize}
    \item 13 hip\footnote{highly interesting person} junior researchers (from within 1 year of graduation with a PhD up to 1 year after reaching tenure at a university of equivalent in industry)
    \item 3 hip senior researchers  (note each individual can only partake in this role at a HIPstIR once in their lifetime)
    \item 3 hip software developers or consultants (interested, but not necessarily focused on IR)
    \item 3 dedicated organizers (a local chair, an agenda chair, and an all-of-the-above chair)
    \item a hip\footnote{highly inspiring place} town to meet
    \item hip locations to congregate during three days
    \item plenty of hip\footnote{high in protein} food and drinks (and after hour locations)
    \item a fun and hip\footnote{high-intensity program} after-hours activity
    \item 22 clipboards with paper
    \item 50 crayons, glitter glue, and poster paper (cardboard as makeshift easels)
    \item a Slack channel to locate people and track post-event discussions
    \item (to taste) 1-2 sponsors to be able to purchase some food \& stationary in advance  -- Mille Gracie to Microsoft and the ACM SIGIR for their support!
\end{itemize}

\paragraph{Party Invites:}

Set a date and location, then invite your researchers. (Be prepared for cancellation, maintain a wait list, ask participants for dietary restrictions, and identify junior researchers that are in need to travel support)

\paragraph{Pre-meeting homework:}

Ask every participant to prepare a pitch with hip title and abstract. Also ask for a list of papers that might lead to new topics, preferably papers that would go unnoticed otherwise.

\paragraph{HIPstIR meeting, round 1 "the pitches" (2.5 h, sitting in a circle):}

Every participant introduces themselves and their pitch ("2" minutes each --- which translates into 6 minutes in human time). questions and cross-references are explicitly desired. Pitches and topics are allowed to change anytime. Spontaneous group formation and merges are welcome!

Each participants name two participants they want to talk to throughout the rest of the night. (These are noted on the "chart of commitment")

\paragraph{HIPstIR meeting, round 2 "the group formation" (2.5 h, standing up): }

Each participant writes three words about their pitch on their clipboard, holding it up. Each pitch is briefly recapped (20 seconds max). Participants move next to one another when pitches are related.

After all pitches have been recapped, the radius of the circle is increased, groups are encouraged to find themselves, and decide a topic. Five groups are preferred. The group topic is written on a clip board and held up for everyone to see. People are allowed to change groups any time, group topics are allowed to change any time.


\paragraph{HIPstIR meeting, round 3 "group discussion and poster" (4h in breakout groups, group changes possible):}

Each group is asked to discuss and flesh out their topics: Define the topic, give an example, identify the challenges, potentially identify an approach to solve the challenges. The group uses their crayons and glitter glue to design a poster for the next day.

\paragraph{HIPstIR meeting, round 4: "The surprise challenge" (varies, small groups transitioning to a plenary discussion):}

Pose a challenge to all participants. In the first installment of HIPstIR, the challenge was to identify a  backronym for "HIPstIR", we collected suggestions from individuals and small groups on a poster and discussed and voted on the options over dinner. 

\paragraph{HIPstIR meeting, round 5: "After hours" (varies, all together):}

Provide a hip\footnote{highly inspiring place} hangout spot for participants to socialize after the hard day of work (in the first installment of HIPstIR we had a fire at the beach and made fire corn on the cob).

\paragraph{HIPstIR meeting, round 6: "The poster session" (3h, sitting in an open space, such as a park):}

Every group presents their poster to everyone. Impromptu discussions are encouraged if not too long. Every group names an ambassador who takes responsibility for writing an abstract. Any participant can indicate interest in any group (multiple expressions possible).

Official closing (distribute feedback form) and take a hip\footnote{how I propose} picture (hipp). But that does not mean it is over yet...

\paragraph{HIPstIR meeting, round 7: "Cool down and discuss" (varies):}

Encourage participants to stay for a little longer, finish any unstructured discussions that they started, have people reflect on the event, hang out and cool down after this high-intensity program (hip).

\paragraph{Post-meeting: "Group abstracts and proposal writing" (distributed):}

Each group writes a two-paragraph abstract about their topic. These abstracts will become part of the HIPstIR report. The goal of the group is to write workshop proposals, grants, and papers. These are the true outcomes of the HIPstIR (the report is just for entertainment and transparency). Ask participants to acknowledge HIPstIR upon successful workshop proposals, papers, and grants.

\paragraph{Epilogue.}

Organizers write a HIPstIR report, to be published in SIGIR Forum. Include group abstracts, pictures of posters, the hip people picture, and some advice for the next organizers. Then encourage more HIPstIRs to be organized in different regions, different seasons, and in different time zones. 




































